Modified Frank-Wolfe Algorithm for Enhanced Sparsity in Support Vector Machine Classifiers

This work proposes a new algorithm for training a re-weighted L2 Support Vector Machine (SVM), inspired on the re-weighted Lasso algorithm of Cand\`es et al. and on the equivalence between Lasso and SVM shown recently by Jaggi. In particular, the margin required for each training vector is set independently, defining a new weighted SVM model. These weights are selected to be binary, and they are automatically adapted during the training of the model, resulting in a variation of the Frank-Wolfe optimization algorithm with essentially the same computational complexity as the original algorithm. As shown experimentally, this algorithm is computationally cheaper to apply since it requires less iterations to converge, and it produces models with a sparser representation in terms of support vectors and which are more stable with respect to the selection of the regularization hyper-parameter.

==> Definitions.tex <==
\RequirePackage{luatex85,shellesc} % For TL 2016.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DEFINITIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Configuration.
    % Theorems.
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem*{lemma}{Lemma}
    % References.
\AfterEndPreamble{\let\ref\cref\undef{\cref}\undef{\autoref}\let\Ref\Cref\undef{\Cref}}
\Crefname{equation}{}{}\crefname{equation}{}{}
\Crefname{figure}{Fig.}{Figs.}\crefname{figure}{Fig.}{Figs.}
\Crefname{problem}{Problem}{Problems}\crefname{problem}{Problem}{Problems}\creflabelformat{problem}{#2\textup{(#1)}#3}
\Crefname{case}{Case}{Cases}\crefname{case}{Case}{Cases}\creflabelformat{case}{#2#1#3}
\Crefname{algorithm}{Algorithm}{Algorithms}\crefname{algorithm}{Alg.}{Algs.}
\Crefname{line}{Line}{Lines}\crefname{line}{Line}{Lines}
\Crefname{mlemma}{Lemma}{Lemmas}\crefname{mlemma}{Lemma}{Lemmas}
\Crefname{mtheor}{Theorem}{Theorems}\crefname{mtheor}{Theorem}{Theorems}
    % Debug.
\overfullrule=10mm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Fonts.
\usepackage[scaled=0.86]{helvet}
% Figures.
    % Colours.
\colorlet{graphic1}{MidnightBlue}
\colorlet{graphic3}{Goldenrod!80!Black}
\colorlet{graphic5}{BrickRed}
\colorlet{graphic7}{Fuchsia}
\colorlet{graphic2}{graphic1!50!graphic3}
\colorlet{graphic4}{graphic3!50!graphic5}
\colorlet{graphic6}{graphic5!50!graphic7}
\colorlet{graphic8}{graphic7!50!graphic1}
\colorlet{colorda}{Green}
\colorlet{colordb}{Dandelion}
\colorlet{colordc}{Red}
\colorlet{mycolor1}{graphic1}
\colorlet{mycolor2}{graphic5}
\colorlet{box}{graphic3!20}
\colorlet{boxo}{graphic1!20}
\colorlet{boxm}{graphic5!20}
\colorlet{arrowc}{graphic5}
    % Figures.
\newif\ifusetikz\usetikztrue
\usetikzfalse
\usetikzlibrary{external}
\usetikzlibrary{patterns}
\usetikzlibrary{arrows}
\tikzexternalize[prefix=./]
\DeclareGraphicsExtensions{.pdf}
\graphicspath{{../}}
%\pgfplotsset{compat=1.15}
\pgfplotsset{colormap={graphicmap}{color=(graphic1) color=(graphic3) color=(graphic5)}}
\pgfplotsset{every axis plot/.append style={line width=1pt}}
\pgfplotsset{scale only axis}
    % Commands.
\newcommand{\includetikz}[1]{\ifusetikz\begin{minipage}{\figwidth}\vspace{0pt}\scriptsize\tikzsetnextfilename{#1}{\tikzset{trim axis left,trim axis right}\input{./#1.tikz}}\end{minipage}\else\includegraphics{#1.pdf}\fi}
\newcommand{\includetikzna}[1]{\ifusetikz\scriptsize\tikzsetnextfilename{#1}{\input{./#1.tikz}}\else\includegraphics{#1.pdf}\fi}

\newcommand{\includetikzfk}[1]{\begin{minipage}{\columnwidth}\scriptsize{#1}\end{minipage}}
\newcommand{\figwidth}{\textwidth}
\newcommand{\tikzwidth}[1]{\renewcommand{\figwidth}{#1}}
\newcommand{\smallmarks}{1pt}
\newcommand{\largemarks}{5pt}
\newcommand{\largelines}{1pt}
\newcommand{\mycaption}{}
\newenvironment{mfiguretikz}[1]{\renewcommand{\mycaption}{#1}\begin{figure}[!tb]\begin{center}\begin{minipage}{0.8\columnwidth}\begin{center}}{\end{center}\end{minipage}\caption[PDFCaption]{\mycaption}\end{center}\end{figure}}
\newenvironment{mfigurepdf}[1]{\renewcommand{\mycaption}{#1}\begin{figure}[!tb]\begin{center}}{\end{center}\caption[PDFCaption]{\mycaption}\end{figure}}
\newenvironment{mfigure}[1]{\ifusetikz\begin{mfiguretikz}{#1}\else\begin{mfigurepdf}{#1}\fi}{\ifusetikz\end{mfiguretikz}\else\end{mfigurepdf}\fi}
\newenvironment{mfiguretikzl}[1]{\renewcommand{\mycaption}{#1}\begin{figure}[p]\begin{center}\begin{minipage}{0.8\columnwidth}\begin{center}}{\end{center}\end{minipage}\caption[PDFCaption]{\mycaption}\end{center}\end{figure}}
\newenvironment{mfigurepdfl}[1]{\renewcommand{\mycaption}{#1}\begin{figure}[p]\begin{center}}{\end{center}\caption[PDFCaption]{\mycaption}\end{figure}}
\newenvironment{mfigurel}[1]{\ifusetikz\begin{mfiguretikzl}{#1}\else\begin{mfigurepdfl}{#1}\fi}{\ifusetikz\end{mfiguretikzl}\else\end{mfigurepdfl}\fi}
\newenvironment{mfigurec}[1]{\renewcommand{\mycaption}{#1}\begin{figure*}[!tb]\begin{center}}{\caption[PDFCaption]{\mycaption}\end{center}\end{figure*}}
\newcommand{\mincludegraphics}[1]{\raisebox{-\height}{\includegraphics{./#1.pdf}}}
\newcommand{\mincludegraphicspng}[2]{\includegraphics[scale=#2]{./#1.png}}
\newcommand{\plotline}{}
\newcommand{\plotarea}{}
\newcommand{\showlegend}[1]{\raisebox{2\height}{\plotline{#1}}}
\newcommand{\showlegendcolour}[1]{\tikzset{external/export next=false}\tikz{\node[draw=black,fill=#1,minimum size=4pt] {};}}
\newcommand{\showlegenddouble}[2]{\makebox[0pt][l]{\plotarea{#1}}\raisebox{2\height}{\plotline{#2}}}
\newcommand{\figsep}{\,}
\newcommand{\figformattitle}[1]{\textbf{\boldmath{#1}}}
\newcommand{\figvsep}{\\\vspace{0pt}\\}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithms.
\newenvironment{malgorithm}[1]{\begin{algorithm}[!tb]\caption{#1}\footnotesize}{\end{algorithm}}
\newcommand{\colorcomment}{Gray}
\algrenewcommand{\algorithmiccomment}[1]{\hfill{\color{\colorcomment}\scriptsize$\blacktriangleright$ \begin{minipage}{0.3\linewidth}{\strut\textit{#1}}\end{minipage}}}
\newcommand{\algorithmiccommentb}[1]{\Statex{\color{\colorcomment}\textit{#1}}}
\newcommand{\algorithmiccommentl}[1]{\Statex{\color{\colorcomment}\dotfill\textit{#1}\dotfill}}
\algnewcommand\algorithmictake{\textbf{set}}
\algnewcommand\Take{\State \algorithmictake~}
\algrenewcommand\alglinenumber[1]{\tiny #1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tables.
\newcommand{\tablesep}{\midrule}
\newcommand{\tableempty}{\ensuremath{\times}}
\newcommand{\tabformathrow}[1]{\textbf{\boldmath{#1}}}
\setlength{\tabcolsep}{4pt}
\newcommand{\sizetitle}{25pt}
\newcommand{\datasettitle}[1]{\multirow{2}{*}{\truncate[]{\sizetitle}{#1}\,$\Bigl\{$}}
\newenvironment{mtable}[1]{\renewcommand{\mycaption}{#1}\begin{table}[!tb]\begin{center}\scriptsize\begin{center}}{\end{center}\end{center}\caption[PDFCaption]{\mycaption}\end{table}}
\newenvironment{mtablel}[1]{\renewcommand{\mycaption}{#1}\begin{table}[p]\begin{center}\tiny\begin{center}\def\arraystretch{0.9}}{\end{center}\end{center}\caption[PDFCaption]{\mycaption}\end{table}}

%\def\arraystretch{0.8}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definitions.
    % Mathematics.
\newcommand{\set}[1]{\{#1\}}
\newcommand{\setst}[2]{\set{#1 \mid #2}}
\newcommand{\sign}[1]{\operatorname{sgn}\prn{#1}}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\diag}{diag}
\newcommand{\minv}[1]{#1^{-1}}
\newcommand{\lagr}{\mathcal{L}}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\sfrac}[2]{#1 / #2}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\mine}[1]{\min\cbr{#1}}
\newcommand{\maxe}[1]{\max\cbr{#1}}
\newcommand{\minme}[1]{\min\{#1\}}
\newcommand{\maxme}[1]{\max\{#1\}}
        % Norms.
\newcommand{\lpg}[1]{\ensuremath{\ell_{#1}}}
\newcommand{\lp}{\lpg{p}}
\newcommand{\lpp}{\ensuremath{\lpg{p}^ p}}
\newcommand{\lz}{\lpg{0}}
\newcommand{\lo}{\lpg{1}}
\newcommand{\lt}{\lpg{2}}
\newcommand{\lto}{\lpg{2,1}}
\newcommand{\lti}{\lpg{2,\infty}}
\newcommand{\loi}{\lpg{1,\infty}}
\newcommand{\np}[1]{\left \| #1 \right \|_p}
\newcommand{\npp}[1]{\np{#1}^p}
\newcommand{\nz}[1]{\left \| #1 \right \|_0}
\newcommand{\no}[1]{\left \| #1 \right \|_1}
\newcommand{\nt}[1]{\left \| #1 \right \|_2}
\newcommand{\nto}[1]{\left \| #1 \right \|_{2,1}}
\newcommand{\nin}[1]{\left \| #1 \right \|_\infty}
\newcommand{\ntin}[1]{\left \| #1 \right \|_{2,\infty}}
\newcommand{\nn}[1]{\left \| #1 \right \|_*}
\newcommand{\nf}[1]{\left \| #1 \right \|_\text{F}}
        % Optimization.
\newcommand{\agropt}[1]{\left \{ #1 \right \}}
\newcommand{\sepopt}{~}
\newcommand{\sepcon}{\enspace}
\newcommand{\sepeq}{\quad ; \quad}
\newcommand{\sepim}{\quad \implies \quad}
\newcommand{\sepcons}{,\sepcon}
\newcommand{\minp}[2]{\min_{#1}\sepopt{\agropt{#2}}}
\newcommand{\minpc}[3]{\min_{#1}\sepopt{\agropt{#2}}\sepcon\text{s.t.}\sepcon #3}
\newcommand{\minpcl}[3]{\min_{#1}\sepopt{\agropt{#2}}\sepcon\text{s.t.}\sepcon \begin{array}[t]{rcl}#3\end{array}}
\newcommand{\argminp}[2]{\arg\min_{#1}\sepopt{\agropt{#2}}}
\newcommand{\argminpc}[3]{\arg\min_{#1}\sepopt{\agropt{#2}}\sepcon\text{s.t.}\sepcon #3}
\newcommand{\argminpcd}[3]{\begin{array}[t]{l}\displaystyle\arg\min_{#1}\sepopt{\agropt{#2}}\\\text{s.t.}\sepcon #3\end{array}}
\newcommand{\opts}{\star}
\newcommand{\opt}[1]{#1^\opts}
         % Utils.
\newcommand{\msfrac}[2]{#1 / #2}
    % Constants.
\newcommand{\npat}{N}
\newcommand{\npatp}{\npat'}
\newcommand{\ndim}{D}
\newcommand{\nout}{P}
\newcommand{\ndimb}{{\bar{D}}}
\newcommand{\ndimn}[1]{D_{#1}}
\newcommand{\ndimg}{D_g}
\newcommand{\ndimv}{D_v}
\newcommand{\ndimo}{D_1}
\newcommand{\ndimt}{D_2}
\newcommand{\ndimp}{\bar{D}}
\newcommand{\ndimgp}{\bar{D}_g}
\newcommand{\nedge}{L}
\newcommand{\preg}{\ensuremath{\lambda}}
\newcommand{\pcon}{\ensuremath{\rho}}
\newcommand{\degp}{N}
    % Sets.
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rd}{\R^\ndim}
\newcommand{\Rdb}{\R^\ndimb}
\newcommand{\Rtd}{\R^{2 \ndim}}
\newcommand{\Rdot}{\R^{\ndimo \times \ndimt}}
\newcommand{\Rdo}{\R^{\ndim \times \nout}}
\newcommand{\Rdos}{\R^{\ndim \cdot \nout}}
\newcommand{\Rdm}{\R^{\ndim - 1}}
\newcommand{\Rdtm}{\R^{\ndim - 2}}
\newcommand{\Rdp}{\R^{\ndimp}}
\newcommand{\Rp}{\R^\npat}
\newcommand{\Rpp}{\R^{\npat \times \npat}}
\newcommand{\Rdd}{\R^{\ndim \times \ndim}}
\newcommand{\Rpd}{\R^{\npat \times \ndim}}
\newcommand{\Rpo}{\R^{\npat \times \nout}}
    % Utils.
\newcommand{\half}{\frac{1}{2}}
\newcommand{\tr}{\intercal}
\newcommand{\dimm}[2]{{#1}^{\prn{#2}}}
\newcommand{\cmp}[2]{#1_{#2}}
\newcommand{\cmpv}[2]{#1_{\brq{#2}}}
\newcommand{\kron}[2]{#1 \otimes #2}
\newcommand{\prn}[1]{{\left ( #1 \right )}}
\newcommand{\prns}[1]{{( #1 )}}
\newcommand{\brq}[1]{{\left [ #1 \right ]}}
\newcommand{\cbr}[1]{{\left \{ #1 \right \}}}
\newcommand{\eeq}[1]{\, #1}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\newcommand{\inter}[1]{\brq{#1}}
\newcommand{\interco}[1]{\left [ #1 \right )}
\newcommand{\hadam}{\circ}
    % Variables.
\newcommand{\mz}{\ensuremath{\mathbf{Z}}}
\newcommand{\mk}{\ensuremath{\mathbf{K}}}
\newcommand{\mkh}{\ensuremath{\hat{\mk}}}
\newcommand{\vkh}{\ensuremath{\mathbf{\hat{k}}}}
\newcommand{\skh}{\ensuremath{\hat{k}}}
\newcommand{\mkhi}[1]{\ensuremath{\vkh_{#1}}}
\newcommand{\vkhi}[1]{\ensuremath{\skh_{#1}}}
\newcommand{\vz}{\ensuremath{\mathbf{z}}}
\newcommand{\vg}{\ensuremath{\mathbf{g}}}
\newcommand{\vgi}[1]{\ensuremath{g_{#1}}}
\newcommand{\vdir}{\ensuremath{\mathbf{d}}}
\newcommand{\vdiri}[1]{\ensuremath{d_{#1}}}
\newcommand{\bas}[1]{\ensuremath{\mathbf{e}_{#1}}}
\newcommand{\mzi}[1]{\ensuremath{\vz_{#1}}}
\newcommand{\mx}{\ensuremath{\mathbf{X}}}
\newcommand{\mxt}{\bar{\mx}}
\newcommand{\mxtt}{\bar{\mxt}}
\newcommand{\mxi}[1]{\ensuremath{\vx_{:,#1}}}
\newcommand{\mxp}[1]{\ensuremath{\vx_{#1}}}
\newcommand{\vx}{\ensuremath{\mathbf{x}}}
\newcommand{\sx}{\ensuremath{x}}
\newcommand{\sxh}{\ensuremath{\hat{x}}}
\newcommand{\sxt}{\ensuremath{\tilde{x}}}
\newcommand{\my}{\ensuremath{\mathbf{Y}}}
\newcommand{\vy}{\ensuremath{\mathbf{y}}}
\newcommand{\sy}{\ensuremath{y}}
\newcommand{\vyt}{\bar{\vy}}
\newcommand{\vytt}{\bar{\vyt}}
\newcommand{\myi}[1]{\ensuremath{\vy_{#1}}}
\newcommand{\vyi}[1]{\ensuremath{\sy_{#1}}}
\newcommand{\vyio}[2]{\ensuremath{\sy_{#1}^{#2}}}
\newcommand{\sys}{\ensuremath{y^*}}
\newcommand{\mw}{\ensuremath{\mathbf{W}}}
\newcommand{\vw}{\ensuremath{\mathbf{w}}}
\newcommand{\vwt}{\bar{\vw}}
\newcommand{\sw}{\ensuremath{w}}
\newcommand{\vwi}[1]{\ensuremath{\sw_{#1}}}
\newcommand{\vwik}[2]{\ensuremath{\sw_{#1}^{(#2)}}}
\newcommand{\vwk}[1]{\ensuremath{\vw^{(#1)}}}
\newcommand{\mwi}[1]{\ensuremath{\vw_{#1}}}
\newcommand{\mt}{\ensuremath{\mathbf{T}}}
\newcommand{\vt}{\ensuremath{\mathbf{t}}}
\newcommand{\st}{\ensuremath{t}}
\newcommand{\vti}[1]{\ensuremath{\st_{#1}}}
\newcommand{\vtik}[2]{\ensuremath{\st_{#1}^{(#2)}}}
\newcommand{\vtk}[1]{\ensuremath{\vt^{(#1)}}}
\newcommand{\va}{\ensuremath{\boldsymbol{\alpha}}}
\newcommand{\vak}[1]{\ensuremath{\boldsymbol{\alpha}^{(#1)}}}
\newcommand{\vaok}[1]{\va^{\opts(#1)}}
\newcommand{\vaiok}[2]{\vai{#1}^{\opts(#2)}}
\newcommand{\sa}{\ensuremath{\alpha}}
\newcommand{\vai}[1]{\ensuremath{\sa_{#1}}}
\newcommand{\vaik}[2]{\ensuremath{\sa_{#1}^{(#2)}}}
\newcommand{\vbe}{\ensuremath{\mathbf{b}}}
\newcommand{\sbe}{\ensuremath{b}}
\newcommand{\vbei}[1]{\ensuremath{\sbe_{#1}}}
\newcommand{\scs}{\ensuremath{s}}
\newcommand{\scb}{\ensuremath{b}}
\newcommand{\vb}{\ensuremath{\mathbf{\scb}}}
\newcommand{\vbi}[1]{\ensuremath{\scb_{#1}}}
\newcommand{\vv}{\ensuremath{\mathbf{v}}}
\newcommand{\mvi}[1]{\ensuremath{\vv_{#1}}}
\newcommand{\vei}[1]{\ensuremath{\mathbf{e}_{#1}}}
\newcommand{\vze}{\ensuremath{\mathbf{0}}}
\newcommand{\von}{\ensuremath{\mathbf{1}}}
\newcommand{\mmx}{\ensuremath{\mathbf{X}}}
\newcommand{\mmxi}[1]{\ensuremath{\mmx_{#1}}}
\newcommand{\vdi}[1]{\ensuremath{\mathbf{p}_{#1}}}
\newcommand{\vdio}[2]{\ensuremath{\mathbf{p}_{#1}^{#2}}}
\newcommand{\iden}[1]{\ensuremath{\mathbf{I}_{#1}}}
\newcommand{\md}{\ensuremath{\mathbf{P}}}
\newcommand{\mq}{\ensuremath{\mathbf{Q}}}
\newcommand{\act}{\ensuremath{\mathcal{W}}}
\newcommand{\acto}{\ensuremath{\opt{\act}}}
\newcommand{\tset}{\ensuremath{\mathcal{T}}}
\newcommand{\ina}{\ensuremath{\bar{\act}}}
\newcommand{\actk}[1]{\ensuremath{\act^{(#1)}}}
\newcommand{\inar}{\ensuremath{\bar{\act}_\text{r}}}
\newcommand{\upd}{\ensuremath{\mathcal{U}}}
\newcommand{\fchn}{b_\text{chng}}

\newcommand{\gap}{\ensuremath{\delta}}
\newcommand{\fobj}{\ensuremath{f}}
\newcommand{\stpg}{\ensuremath{\gamma}}

\newcommand{\fmon}{\ensuremath{f_\text{mon}}}

\newcommand{\massk}[1]{m^{(#1)}}

\newcommand{\ndeac}{d}
    % Comments.
\newcommand{\comr}[1]{{\color{Red}#1}}
\newcommand{\comb}[1]{{\color{Blue}#1}}
\newcommand{\comg}[1]{{\color{Green}#1}}
\newcommand{\comm}[1]{\comb{#1}}
\newcommand{\comj}[1]{\comr{JS: #1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Formats.
\setlength{\fboxsep}{2pt}
\newcommand{\formatany}[2]{{\colorbox[HTML]{#2}{\color{Black}\makebox[\widthbox][c]{\raisebox{0pt}[\height][0pt]{#1}}}}}
\newcommand{\widthbox}{}
\newcommand{\formata}[1]{\formatany{#1}{31a354}}
\newcommand{\formatb}[1]{\formatany{#1}{a1d99b}}
\newcommand{\formatc}[1]{\formatany{#1}{e5f5e0}}
% #e5f5e0 #a1d99b #31a354
% #edf8e9 #bae4b3 #74c476 #238b45
% #edf8e9 #bae4b3 #74c476 #31a354 #006d2c
\newcommand{\vertcell}[1]{\rotatebox[origin=c]{90}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Models and Datasets.
\newcommand{\formatm}[1]{\textsf{#1}}
\newcommand{\isvmname}{SVM\textsuperscript{\mfw{}}}
\newcommand{\ssvm}{\formatm{SVM}}
\newcommand{\isvm}{\formatm{\isvmname}}
\newcommand{\fisvm}{\formatm{SVM$^\text{\mfw{}}_\text{FP}$}}

\newcommand{\formatd}[1]{\texttt{#1}}
\newcommand{\daust}{\formatd{australian}}
\newcommand{\dbrea}{\formatd{breast}}
\newcommand{\ddiab}{\formatd{diabetes}}
\newcommand{\dgerm}{\formatd{german}}
\newcommand{\dhear}{\formatd{heart}}
\newcommand{\diono}{\formatd{ionosphere}}
\newcommand{\diris}{\formatd{iris}}
\newcommand{\dmini}{\formatd{miniboone}}
\newcommand{\dmush}{\formatd{mushrooms}}
\newcommand{\dsona}{\formatd{sonar}}
\newcommand{\dijcn}{\formatd{ijcnn}}
\newcommand{\dmgam}{\formatd{mgamma}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithms.
\newcommand{\fw}{FW}
\newcommand{\mfw}{M-\fw}
\newcommand{\rwla}{RW-Lasso}
\newcommand{\wsvm}{W-SVM}
\newcommand{\rwsvm}{RW-SVM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Others.
\newcommand{\largefigure}{190pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Biography.
\newcommand{\fbook}[1]{``#1''}
\newcommand{\fjournal}[1]{``#1''}
\newcommand{\fconf}[1]{\emph{#1}}
\newcommand{\fsoc}[1]{\emph{#1}}

% Emails.
\newcommand{\email}[1]{\href{mailto:#1}{#1}}

% Legends.
\newlength{\lenaux}
%\newcommand{\legend}[2]{\scriptsize\settowidth{\lenaux}{#1}\hfill\fbox{\begin{minipage}{\lenaux}#2\end{minipage}}\\\vspace{5pt}}
\newcommand{\legend}[2]{\scriptsize\fbox{#2}\\\vspace{5pt}}
%\newcommand{\seplegend}{\\}
\newcommand{\seplegend}{\qquad}

% Emails.
\newcommand{\showemail}[1]{Email: \email{#1}.}
